Anomaly Detection and Localization for Speech Deepfakes via Feature Pyramid Matching

The rise of AI-driven generative models has enabled the creation of highly realistic speech deepfakes - synthetic audio signals that can imitate target speakers' voices - raising critical security concerns. Existing methods for detecting speech deepfakes primarily rely on supervised learning, which suffers from two critical limitations: limited generalization to unseen synthesis techniques and a lack of explainability. In this paper, we address these issues by introducing a novel interpretable one-class detection framework, which reframes speech deepfake detection as an anomaly detection task. Our model is trained exclusively on real speech to characterize its distribution, enabling the classification of out-of-distribution samples as synthetically generated. Additionally, our framework produces interpretable anomaly maps during inference, highlighting anomalous regions across both time and frequency domains. This is done through a Student-Teacher Feature Pyramid Matching system, enhanced with Discrepancy Scaling to improve generalization capabilities across unseen data distributions. Extensive evaluations demonstrate the superior performance of our approach compared to the considered baselines, validating the effectiveness of framing speech deepfake detection as an anomaly detection problem.

==> old_text/1_introduction_old.tex <==
\section{Introduction}

In recent years, the rapid advancement of AI-driven generative systems has made the creation of high-quality synthetic multimedia content easier than ever.
However, this democratization of generative systems carries significant societal risks, as malicious actors could exploit these tools to create deceptive synthetic media, for identity theft, financial fraud, and disinformation campaigns~\cite{amerini2024deepfake}.

In the audio domain, among these threats we can find speech deepfakes, synthetic-generated audio that mimics a target speaker’s voice making them say arbitrary utterances. 
These synthetic audio samples can be exploited to fabricate deceptive communications, leading to cases of fraud, blackmail, and other security threats. To mitigate these risks, the multimedia forensics community has actively developed deepfake detection systems aimed at preserving the integrity of digital communications.

Various approaches have been proposed for speech deepfake detection, ranging from the analysis of low-level acoustic features~\cite{sahidullah2015comparison, pal2018synthetic} to the examination of higher-level speech characteristics~\cite{conti2022deepfake}. These methods employ diverse architectures, spanning from traditional machine learning techniques to advanced deep learning models and pre-trained systems.
Most existing detection systems adopt a supervised learning paradigm, where models are trained on labeled datasets comprising both real and synthetic speech samples.
However, this approach presents two key challenges: generalization and interpretability. Generalization refers to the model's ability to effectively detect deepfakes generated by previously unseen speech synthesis algorithms, a limitation that can compromise its robustness in real-world scenarios.
Interpretability, on the other hand, concerns the black-box nature of these models, which often provide little insight into the underlying reasoning behind their predictions. 

To address these challenges, recent efforts have explored unsupervised learning and, more specifically, \gls{occ}-based methods as an alternative approach for \gls{sdd}.
In \gls{occ}, the model learns to characterize the distribution of normal data (i.e. genuine speech) and establishes a boundary around it. Any samples falling outside this boundary are then flagged as anomalous cases\cite{kim2024one}. \\

Also referred to as outlier or novelty detection, \gls{ad} is generally understood  as the process of identifying rare instances of data (events or observations) that significantly deviate from a well-defined notion of normal behavior, namely anomalies \cite{chandola2009anomaly}. Since labeled data is often unavailable in standard \gls{ad} settings, \gls{occ}-based methods are the predominant approach for this task. \\

The relationship between \gls{sdd} and \gls{ad} lies in the nature of synthetic speech. Signals generated or manipulated artificially inevitably contain artifacts, which can be seen as anomalies within the distribution of genuine speech. 
When extended to \gls{al}, the objective is not only to detect suspicious patterns within the speech data distribution but also to pinpoint the temporal and/or spectral regions where the anomaly occurs within potentially manipulated speech. This localization provides detailed insights into the onset, duration, and frequency characteristics of the anomalous events, enhancing the explainability of the detection process.\\

Motivated by this, we build upon the work of Valjakka et al. \cite{valjakka2023anomaly}, who successfully applied the \gls{stfpm} \cite{wang2021student_teacher} framework to perform \gls{ad} and \gls{al} in a controlled scenario, and adapt this approach to the challenge of \gls{sdd}. Originally developed for \gls{ad} and \gls{al} in images, the \gls{stfpm} is a \gls{occ}-based method employing a feature pyramid matching strategy to capture anomalies at different levels of resolution. By doing so, the authors effectively manage to detect anomalies at both pixel (more subtle) and image level (large scale). This paper proposes an adaptation of the \gls{stfpm} framework to evaluate the effectiveness of the feature pyramid matching approach in identifying and localizing anomalies in time-frequency representations of speech signals, likely indicators of artificially induced artifacts, across different scenarios.\\




==> old_text/2_method_old.tex <==
\section{Proposed Method}
\label{sec:method}

In this section, we begin by formulating the problem at hand, then we continue by presenting the method we propose to address such problem, highlighting the rationale behind our hypotheses. 

% COPIATO E INCOLLATO
% Motivated by this, we build upon the work of Valjakka et al. \cite{valjakka2023anomaly}, who successfully applied the \gls{stfpm} \cite{wang2021student_teacher} framework to perform \gls{ad} and \gls{al} in a controlled scenario, and adapt this approach to the challenge of \gls{sdd}. Originally developed for \gls{ad} and \gls{al} in images, the \gls{stfpm} is a \gls{occ}-based method employing a feature pyramid matching strategy to capture anomalies at different levels of resolution. By doing so, the authors effectively manage to detect anomalies at both pixel (more subtle) and image level (large scale). This paper proposes an adaptation of the \gls{stfpm} framework to evaluate the effectiveness of the feature pyramid matching approach in identifying and localizing anomalies in time-frequency representations of speech signals, likely indicators of artificially induced artifacts, across different scenarios.\\

\subsection{Problem Formulation}
\label{subsec:problem}
The \gls{sdd} problem can be formally defined as follows. 
Let us consider a discrete-time input speech signal $\mathbf{x}$ associated with a class $y \in \{0, 1\}$, where \num{0} denotes that the signal is authentic and \num{1} indicates that it has been synthetically generated.
The goal of this task is to develop a detector $\mathcal{D}$ that is able to estimate the class of the signal $\mathbf{x}$ as $\hat{y} \in [0,1]$, where $\hat{y}$ is the likelihood of the signal $\mathbf{x}$ being fake.

In this work, following an \gls{ad} approach, we address the problem in a one-class fashion, where $\mathcal{D}$ is trained to model the distribution of genuine speech. 
The likelihood $\hat{y}$ is then interpreted as a measure of deviation from this distribution, with higher values indicating a greater likelihood of the signal being synthetic.


\subsection{Proposed System}
\label{subsec:system}

We reframe the \gls{sdd} task as one of \gls{ad} and \gls{al}.
Given a speech signal under analysis, our objective is to determine whether it exhibits 
%acoustic 
patterns that deviate significantly from those that characterize genuine speech.
If that is the case, we also aim to locate the specific time-frequency regions within the audio signal where these potential anomalies, i.e., generation artifacts, occur.

We do so by following an unsupervised \gls{occ} approach in which our system $\mathcal{D}$ learns to model the distribution of genuine speech data only.
The rationale behind this approach is that synthetic speech often introduces subtle yet systematic deviations from the natural speech distribution, regardless of the synthesis method used. 
By focusing only on genuine speech, our system identifies anomalies as deviations from this learned distribution.
This enhances robustness against a wide range of synthesis methods, while completely eliminating the need for synthetic training data.

In this work, we implement $\mathcal{D}$ as a \gls{stm} by adapting the \gls{stfpm} introduced by \cite{wang2021student_teacher}. 
As in the original formulation, our proposed \gls{stfpm} framework exploits a \gls{stm} that consists of a pair of identical \glspl{cnn}-based models.
Likewise, we feed both with the same frequency-domain representations of the speech signal, to enable effective 
visual comparison between the activations of the two networks.

We chose to pre-train the \textit{teacher} model on the speaker identification task. 
The purpose of such a strategy is to force the teacher to learn speech-specific representations, which is crucial to properly address the \gls{sdd} problem at hand.
On the other hand, the \textit{student} network exhibits the same architecture as the teacher, minus the classification layer, as its purpose is to learn to mimic the teacher’s activations.
This is achieved using \gls{fpm} \cite{valjakka2023anomaly}.

\gls{fpm} is a technique to compare the activations of the teacher and student networks at multiple designated layers. 
This allows capturing anomalies at different levels of the network architecture: bottom layers are responsible for encoding low-level information and capturing fine-grained details, whereas top layers extract higher-level information, i.e., the context.
Since the teacher is trained for speaker identification, its activations naturally capture distinctive characteristics of genuine speech. 
As a result, the student network learns to replicate these activations, effectively modeling the distribution of real speech, thus aligning with a \gls{occ} framework.

At inference time, the student can potentially be fed with both real and synthetic data. 
The discrepancy between normalized teacher and student activations is then used as an anomaly indicator.
We will refer to it as \textit{anomaly map}.
If the input speech is genuine, the student will likely replicate the teacher's activations, resulting in small discrepancy values and an anomaly map with no significant deviations. 
However, if the system is presented with synthetic speech, the student 
will struggle to mimic the teacher's activations, leading to larger discrepancy values. 
In principle, areas with higher values on the anomaly map, indicating higher anomaly scores, highlight the time-frequency regions of synthetic speech where generation artifacts are most concentrated.

To further enhance our \gls{stfpm}, we incorporate \gls{ds} \cite{myllari2023discrepancy} to standardize the discrepancy values between the teacher and student networks.
This is achieved at the inference stage, by calculating the mean and standard deviation of the test data distribution. 
These statistics are then used to normalize the discrepancies between teacher and student activations, layer by layer, resulting in an amplification of subtle anomalies.


==> old_text/3_experimental_setup_old.tex <==
\section{Experimental Setup}
\label{sec:setup}

In this section, we outline the evaluation setup employed in our experiments.
We start by detailing the parameters and the strategies that we used to train and evaluate the proposed model.
Then, we introduce the datasets was used for training and testing the \gls{stfpm} framework.
Finally, we present the baseline systems used to validate our results.

\subsection{Training and Evaluation Strategies}

The model that we considered as teacher and student is a modified version of ResNet18~\cite{he2016deep}, trained on Mel-spectrogram inputs with a dropout layer for regularization and a \num{256}-unit ReLU layer for feature extraction.

We used 4-second input audio segments and adjusted the final dense layer of each model to match the number of classes in the classification task.
We trained the models until convergence by monitoring the value of the validation loss, computed via Cross-Entropy function.
We employed cosine annealing for learning rate scheduling and early stopping to prevent overfitting.
We assumed \num{10} epochs as early stopping, a batch size of \num{128}, and a learning rate $lr=$\num{e-4}.

Unlike Valjakka et al.  \cite{valjakka2023anomaly}, who relied on a backbone pre-trained for image classification, we decided to re-train the teacher network on the task of speaker identification.

\textbf{Teacher Network Training.} We trained our teacher network on the task of speaker identification %following a supervised learning approach??. 
For this task, we selected the \textbf{LibriSpeech} dataset \cite{panayotov2015librispeech}, a corpus of read english speech featuring a diverse range of speakers. More specifically, we employed the \textit{train-clean-360} subset, which contains authentic speech from a total of $921$ speakers. From this subset, we retained the first $100$ samples for each speaker and further partitioned them into training ($62962$ utterances) and validation ($26984$ utterances) subsets ensuring a balanced distribution of speakers across the two subsets.\\

%, ending up with $62962$ speech samples for the training set and $26984$ for the validation set. 


%\subsubsection{\textbf{Student Network Training}}
%\label{subsubsec:student training}

\textbf{Student Network Training.} To investigate generalization capabilities of our method, we trained our student network for both single-speaker and multi-speaker scenarios. For our single-speaker model, we selected the LJspeech \cite{ljspeech17} dataset. For our multi-speaker model we employed the \gls{la} partition of the ASVSpoof19 \cite{wang2020asvspoof} dataset.

\begin{itemize}
    \item \textbf{LJspeech}\cite{ljspeech17} is a widely used corpus consisting of $13100$ short audio clips of a single female speaker, totaling approximately $24$ hours of recorded speech. To make our model as less biased as possible, we trained and validated the student excluding tracks later employed in the evaluation step of our model. 
    \item \textbf{ASVspoof19}\cite{wang2020asvspoof} is a benchmark corpus specifically designed for \gls{asv} and SDD. It provides a diverse collection of bona-fide and spoofed speech samples covering various spoofing attacks, from \gls{tts} to \gls{vc}. To train and validate our multi-speaker model, we employed all bona-fide samples from the \textit{train} ($2580$ utterances) and \textit{dev} ($2548$ utterances) subsets of the LA partition, respectively. \\

\end{itemize}


\textbf{Student Network Evaluation.}


\subsection{Datasets}
\label{subsec:dataset}

\noindent\textbf{LibriSpeech~\cite{panayotov2015librispeech}} ($D_\text{LIB}$). \vspace{0.1em} Designed to aid the training and testing of \gls{asr} systems, this corpus contains approximately \num{1000} hours
of speech data from more than \num{200} different speakers. We employ a small subset of its \textit{train-clean-360} partition, which features about \num{360} hours of authentic speech from a total of \num{921} speakers. 

\noindent\textbf{LJ-Speech~\cite{ljspeech17} } ($D_\text{LJ}$).\vspace{0.1em}A dataset comprising \num{13100} genuine speech recordings from a single female speaker reciting passages from non-fictions books, totaling approximately \num{24} hours of audio data. \vspace{0.1em}

\noindent\textbf{Il Nostro :) }\vspace{0.1em}

\noindent\textbf{TIMIT-TTS~\cite{salvi2023timit} ($D_\text{TIM}$)}.
A synthetic speech dataset derived from the VidTIMIT corpus~\cite{sanderson2002vidtimit}. 
We use its \textit{clean} single-speaker partition, which contains speech signals generated using \num{7} \gls{tts} models and replicates the voice of LJSpeech~\cite{ljspeech17}. \vspace{0.1em}
% which contains speech signals generated using \num{12} different \gls{tts} models, with \num{7} dedicated to single-speaker synthesis and \num{5} supporting multiple speakers.
%The single-speaker partition ($D_\text{TIM, SS}$) replicates the voice of LJSpeech~\cite{ljspeech17}, while the multi-speaker partition ($D_\text{TIM, MS}$) synthesizes voices from LibriSpeech~\cite{panayotov2015librispeech}. 

\noindent \textbf{ASVspoof 2019~\cite{wang2020asvspoof}} ($D_\text{ASV}$).
Released for the homonymous challenge, this dataset was designed to develop effective ASV models.
It includes real speech from the VCTK corpus~\cite{veaux2016superseded} and synthetic speech fabricated by \num{19} different synthetic speech generators. 
%Data are distributed unevenly across the dataset partitions to enable open-set evaluation. 
We employ the Logical Access partition of this corpus. \vspace{0.1em}

\noindent\textbf{MLAAD~\cite{muller2024mlaad} ($D_\text{MLA}$)}.
A large-scale dataset that includes synthetic speech signals generated using \num{82} \gls{tts} models, in \num{38} different languages.
\vspace{0.1em}

\noindent \textbf{In-the-Wild~\cite{muller2022does} ($D_\text{ItW}$)}. 
A dataset for evaluating speech deepfake detectors in real-world conditions. 
Fake clips are segmented from public video and audio, while real clips feature the same speakers from publicly available sources.\vspace{0.1em}

\noindent \textbf{Purdue speech dataset~\cite{bhagtani2024recent}} ($D_\text{PUR}$).
This corpus includes \num{25000} synthetic speech tracks generated by \num{5} diffusion model-based voice cloning methods: ProDiff, DiffGAN-TTS, ElevenLabs, UnitSpeech, and XTTS. 
%Real speech data are sourced from LJSpeech~\cite{LJSpeech} and \num{10} speakers from LibriSpeech~\cite{panayotov2015librispeech}.

\noindent \textbf{FakeOrReal~\cite{reimao2019dataset}} ($D_\text{FoR}$).
A dataset of over \num{198000} utterances from real and synthetic speech. 
Synthetic data comes from open-source and commercial \gls{tts} systems, while real data is sourced from diverse open datasets and platforms like TED Talks and YouTube.


\subsection{Baseline systems}


